Unveiling Knowledge Utilization Mechanisms in LLM-based Retrieval-Augmented Generation

Considering the inherent limitations of parametric knowledge in large language models (LLMs), retrieval-augmented generation (RAG) is widely employed to expand their knowledge scope. Since RAG has shown promise in knowledge-intensive tasks like open-domain question answering, its broader application to complex tasks and intelligent assistants has further advanced its utility. Despite this progress, the underlying knowledge utilization mechanisms of LLM-based RAG remain underexplored. In this paper, we present a systematic investigation of the intrinsic mechanisms by which LLMs integrate internal (parametric) and external (retrieved) knowledge in RAG scenarios. Specially, we employ knowledge stream analysis at the macroscopic level, and investigate the function of individual modules at the microscopic level. Drawing on knowledge streaming analyses, we decompose the knowledge utilization process into four distinct stages within LLM layers: knowledge refinement, knowledge elicitation, knowledge expression, and knowledge contestation. We further demonstrate that the relevance of passages guides the streaming of knowledge through these stages. At the module level, we introduce a new method, knowledge activation probability entropy (KAPE) for neuron identification associated with either internal or external knowledge. By selectively deactivating these neurons, we achieve targeted shifts in the LLM's reliance on one knowledge source over the other. Moreover, we discern complementary roles for multi-head attention and multi-layer perceptron layers during knowledge formation. These insights offer a foundation for improving interpretability and reliability in retrieval-augmented LLMs, paving the way for more robust and transparent generative solutions in knowledge-intensive domains.

==> sec/sec-related.tex <==
\newpage

\section{Related Works}

\subsection{Retrieval-Augmented Generation}
Retrieval-augmented generation (RAG) technology first emerged in the application of pre-trained language models~(PLMs)~\cite{lewis2020retrieval}, introduced as a task that jointly trains the generative PLM~(\eg BART~\cite{Lewis2020BARTDS}) with the dense retriever. This approach enabled end-to-end execution of knowledge-intensive tasks that involved retrieval followed by generation.
In the era of large language models~(LLMs)~\cite{zhao2023survey}, the primary focus of RAG research has shifted towards integrating external knowledge sources during the inference stage of LLMs~\cite{gao2023retrieval}. Typically, this is achieved by providing the model with well-designed instructions that incorporate the query and the retrieved documents, allowing the LLM to generate a response by referring to the given documents~\cite{ke2024bridging, ren2023investigating}. Various approaches have been proposed to better leverage the retrieved documents to address the noise present in the retrieved documents. For instance, models may autonomously decide whether to incorporate the retrieved documents~\cite{asaiself}, or reranker models may be jointly trained with the RAG task to improve the model’s relevance perception on the documents and the query~\cite{wang2024rear}.
Furthermore, a brunch of studies focuses on iterative retrieval methods to enhance the quality of search results~\cite{shao2023enhancing}, such as utilizing chain-of-thought reasoning to guide the retrieval process~\cite{trivedi2023interleaving} or employing tree structures to continually refine the query~\cite{kim2023tree}.
RAG also serves as a foundational module to support more complex reasoning tasks~\cite{zhang2023graph}, including solving intricate problems and acting as a knowledge utility for intelligent agents~\cite{wu2024autogen}.
Despite the significant progress made in RAG research, these advancements have predominantly focused on enhancing task-solving capabilities. However, the internal mechanisms governing knowledge utilization within RAG models have not been sufficiently explored, leaving the RAG models largely as black boxes.


\subsection{Interpretation of LLM Mechanisms}

Despite the remarkable success of LLMs across a wide range of natural language processing tasks, the “black-box” nature limits the understanding of their internal behavior, constraining their trustworthiness, particularly in sensitive domains~\cite{zhao2024explainability, huang2023can}. Consequently, substantial research efforts have been devoted to enhancing the interpretability of LLMs, aiming to elucidate the internal logic behind their responses~\cite{bereska2024mechanistic, rai2024practical}.
One branch of LLM interpretability research seeks to analyze the model’s internal mechanisms through observation~\cite{rauker2023toward}, such as perturbing model inputs to observe the influences on neuron activations~\cite{zimmermann2021well} or identifying data points with the strongest influence on specific neurons~\cite{gardedeepdecipher, nanfack2024adversarial}. A representative approach is probing, which involves introducing a classifier to investigate neuron activations~\cite{hewitt2019structural, cao2021low, gurneefinding}. As another notable method, logit lens employs an unembedding strategy to map intermediate hidden states to the final layer’s probability distribution via residual stream accumulation, thereby revealing their impact on model output~\cite{dar2023analyzing, geva2022transformer, atkey2009unembedding}.
Intervention-based methods, on the other hand, actively perturb specific model parameters to uncover causal relationships between parameters and outputs~\cite{mueller2024quest}. A prominent example is the patching method, which modifies intermediate activations to investigate their effect on the model’s reasoning process~\cite{meng2022locating, wanginterpretability, hanna2024does}. Additionally, causal abstraction offers a mathematical framework for explaining internal mechanisms, allowing interpretability analysis from a causal modeling perspective~\cite{geiger2023causal, geiger2024finding}.

Our approach to modeling and analyzing knowledge streaming in RAG draws significant inspiration from the aforementioned interpretability methods. We tailor these methods to suit the characteristics of RAG, enabling rigorous analysis and deeper insights into its functioning.
